In almost all shallow analytic neural network optimization landscapes, efficient minimizers have strongly convex neighborhoods

Whether or not a local minimum of a cost function has a strongly convex neighborhood greatly influences the asymptotic convergence rate of optimizers. In this article, we rigorously analyze the prevalence of this property for the mean squared error induced by shallow, 1-hidden layer neural networks with analytic activation functions when applied to regression problems. The parameter space is divided into two domains: the 'efficient domain' (all parameters for which the respective realization function cannot be generated by a network having a smaller number of neurons) and the 'redundant domain' (the remaining parameters). In almost all regression problems on the efficient domain the optimization landscape only features local minima that are strongly convex. Formally, we will show that for certain randomly picked regression problems the optimization landscape is almost surely a Morse function on the efficient domain. The redundant domain has significantly smaller dimension than the efficient domain and on this domain, potential local minima are never isolated.

==> sections/analytic_norm_response.tex <==
\section{A Criterion for \texorpdfstring{\(\param \mapsto \|\response_\param\|_{\Pr_X}^2\)}{θ → ∥Ψθ∥2} to be analytic}

\begin{prop}[Holomorphic \& bounded response]
    \label{prop: holomorphic and bounded response}
    Let \(\network =(G, \activation, \param)\) be a shallow neural network with
    response function \(\response_\param:\real^{V_\tin}\to\real^{V_\tout}\).
    Assume that the activation function \(\activation\)
    \begin{enumerate}[label=\text{\normalfont(A\arabic*)}]
        \item\label{assmpt: activation is holomorphic}
        is holomorphic on a set which largely excludes the imaginary axis:
        \[
            M := \{ x+ iy : |y| \le c_1(1+|x|)\}\subseteq \complex,
        \]
        for some \(c_1>0\).

        \item\label{assmpt: activation grows at most with power p}
        grows at most with power \(p\ge 0\) on \(M\), i.e. for some \(c_2>0\)
        \[
            |\activation(z)|\le c_2(1+|z|^p)\qquad \forall z\in M.
        \]
    \end{enumerate}
    And assume that the input is one-dimensional, i.e. \(\#V_\tin = 1\).
    Then for any efficient parameter \(\param_*\in \efficient\) there exists a
    compact neighborhood \(K_{\param_*}\subseteq \complex^{\dim(\param_*)}\) such that
    for all \(l\in V_\tout\) 
    \begin{enumerate}[label=\text{\normalfont(R\arabic*)}]
        \item\label{res: response holomorphic}
        the function \(\param \mapsto (\response_\param(x))_l\) is
        holomorphic on \(K_{\param_*}\) for all \(x\in \real^{V_\tin}\).
        \item\label{res: response uniformly bounded}
        If \(X\) has finite \(2p\)-th moment, i.e. \(X\in L^{2p}(\real^{V_\tin})\), 
        there exists \(C_l >0\) such that uniformly over \(\param\in K_{\param_*}\)
        \[
            \int |(\response_\param(x))_l|^2 \Pr_X(dx) < C_l.
        \]
    \end{enumerate}
    In particular, by \ref{res: response holomorphic}, \(\param \mapsto (\response_\param(x))_l\) is real analytic on \(\efficient\).
\end{prop}
\begin{proof}
    The proof has two steps: First, we explain how the results
    follow from the following claim without the assumption of
    one dimensional input (\(|V_\tin|=1\)).
    \begin{claim}\label{claim: inputs in M}
        There exists a compact neighborhood \(K_{\param_*}\) of \(\param_*\)
        (without loss of generality contained in a \(\delta\)-Ball),
        such that for all \(\param\in K_{\param_*}\), we have
        \begin{equation}
            \label{eq: inputs in M}
            \bias_j + \langle x, \weight_{\placeholder j}\rangle \in M
            \qquad
            \forall x\in \real^{V_\tin},\; \forall j\in V_1.
        \end{equation}
    \end{claim}
    In the second step we prove Claim~\ref{claim: inputs in M}, i.e.
    there exists \(K_{\param_*}\), such that Equation~\eqref{eq: inputs in M} is
    satisfied in the case of one dimensional input (\(|V_\tin|=1\))
    and explain why this claim is false without this assumption.

    \paragraph*{Claim~\ref{claim: inputs in M} is sufficient}

    To prove \ref{res: response holomorphic}, i.e. that \(\param\mapsto \response_\param(x)\)
    is holomorphic on \(K_{\param_*}\) for all \(x\in \real^{V_\tin}\),
    it is sufficient to prove that for all
    \(\param \in K_{\param_*}\) we have
    since \(\activation\) is holomorphic on \(M\) and the response
    \(\response_\param\) is simply an affine linear combination of these.
    Furthermore, \eqref{eq: inputs
    in M} together with the assumption \ref{assmpt: activation grows at most with power p} about \(\activation\) also implies the
    uniform bound \ref{res: response uniformly bounded}, since
    \begin{align*}
        |\response_\param(x)|
        &= \Bigl| \bias_l + \sum_{j\in V_1}
        \activation\bigl(
            \bias_j + \langle x, \weight_{\placeholder j}\rangle
        \bigr) \weight_{jl}\Bigr|
        \\
        &\le |\bias_l| + \sum_{j\in V_1}
        \Bigl|\activation\bigl(
            \bias_j + \langle x, \weight_{\placeholder j}\rangle
        \bigr)\Bigr| |\weight_{jl}|
        \\
        \overset{\eqref{eq: inputs in M}, \ref{assmpt: activation grows at most with power p}}&\le
        |\bias_l| + \sum_{l\in V_1}  c_2\bigl(
            1+\bigl|\bias_j + \langle x, \weight_{\placeholder j}\rangle\bigr|^p
        \bigr)|\weight_{jl}|
        \\
        &\le c_l (1+ \|x\|^p)
    \end{align*}
    for some constant \(c_l\) which only depends on \(\param_*\). That is
    because \(\param\) is in a \(\delta\)-Ball around \(\param_*\) so we can
    replace all parameters by the absolute values of \(\theta_*\) plus
    \(\delta\). With the finite \(2p\)-th moment of \(X\),
    \ref{res: response uniformly bounded} immediately follows:
    \[
        \int |(\response_\param(x))_l|^2 \Pr_X(dx)
        \le c_l \int (1 + \|X\|^p )\Pr_X(dx) =: C_l < \infty.
    \]

    \paragraph*{Proof of Claim~\ref{claim: inputs in M}}

    Recall that we need to find a neighborhood \(K_{\param_*}\)
    such that for all \(\param\in K_{\param_*}\) we have uniformly \(\bias_j +
    \langle \weight_{\placeholder j}, x\rangle \in M\).
    By definition of \(M\) we thus need to find some \(c_1>0\)
    such that
    \begin{equation}
        \label{eq: bound im by re}
        \bigl|\Im\bigl(\bias_j + \langle \weight_{\placeholder j}, x\rangle\bigr)\bigr|
        \le c_1\bigl(1+ \bigl|\Re\bigl(\bias_j + \langle \weight_{\placeholder j}, x\rangle\bigr)\bigr|\bigr)
        \qquad \forall x\in \real^{V_\tin},\; \forall j \in V_1,
    \end{equation}
    In this step we will crucially\footnote{
        \textbf{The issue with multiple input dimensions:}
            In the case \(|V_\tin|>1\), there exists a vector
            \(v \perp w_{\placeholder j}^*\). Since \(K_{\param_*}\) has to be a
            neighborhood of \(\param_*\) in \(\complex^{\dim(\param_*)}\),
            there exists some \(\epsilon > 0\) such that
            \(w_{\placeholder j} = w_{\placeholder j}^* + i\epsilon v\)
            is admissible. Assuming (without loss of generality) \(\bias_j\)
            to be equal to zero, we can then chose \(x = \lambda v\) 
            such that for \(\lambda \to \infty\) the imaginary part 
            becomes arbitrarily large, while the real part is zero.  Thus \eqref{eq:
            bound im by re} cannot be satisfied for all \(x\in \real^{V_\tin}\).
    } assume the input to be one-dimensional, i.e. \(|V_\tin| = 1\).
    % It is then convenient to define \(\alpha := \weight_{0 \placeholder}\).
    We define the set \(K_{\param_*}\) explicitly to be
    \begin{align}
        \label{eq: delta w}
        \delta^\weight_j
        &:= \frac{|\weight^*_{\placeholder j}|}2\min\Bigl\{
            1,
            c_1,
            \frac{c_1}{2(1+2|\bias^*_j|)}
        \Bigr\}
        \qquad j\in V_1,
        \\
        \label{eq: delta bias}
        \delta^\bias_j
        &:= \min\Bigl\{\frac{c_1}2, 1+ |\bias^*_j|\Bigr\}
        \qquad j\in V_1,
        \\
        \nonumber
        K_{\param_*} &:= B_{\delta}(\param_*) \cap \Biggl\{
            \param \in \complex^{\dim(\param_*)}:
            |\weight_{\placeholder j} - \weight^*_{\placeholder j}| \le \delta^\weight_j,\;
            |\bias_j - \bias^*_j| \le \delta^\bias_j,\;
            \forall j\in V_1
        \Biggr\}.
    \end{align}

    We will essentially use the fact that \(\param_*\in\efficient\) is real and
    \(\param\) is only allowed to slightly deviate into the complex plane.

    Let \(j\in V_1\) be arbitrary. Our first goal will essentially be to show
    that we can assume \(\bias_j = 0\) without loss of generality.
    For this we define \(x_0\) to be the input where \(\bias_j + \langle \param_{\placeholder j}, x\rangle\)
    is zero. Since we assume \(|V_\tin|=1\) this input can be explicitly
    given by
    \[
        x_0 := -\frac{\Re(\bias_j)}{\Re(\weight_{\placeholder j})}.
    \]
    Let us quickly explain why we do not need to worry about division by zero.
    \(\param_*\) is real and efficient. By Lemma~\ref{lem: general redundancies}
    we thus have \(\weight_{\placeholder j}^* \neq 0\) and by definition of \(\delta_j^{\weight}\)
    we therefore have
    \[
        |\Re(\weight_{\placeholder j})| > |\weight_{\placeholder j}^*| - \delta^\weight_j > \tfrac{|\weight_{\placeholder j}^*|}2 > 0.
    \]
    Let us get back to our original goal to
    set \(\bias_j\) to zero without loss of generality,
    observe that the real part of \(\bias_j + \langle x, \weight_{\placeholder j}\rangle\)
    is given by
    \[
        \Re(\bias_j + \langle x, \weight_{\placeholder j}\rangle)
        = \underbrace{\Re(\bias_j +  \langle x_0, \weight_{\placeholder j}\rangle)}_{=0}
        + \Re(\langle x - x_0, \weight_{\placeholder j}\rangle)
        = \langle  x-x_0, \Re(\weight_{\placeholder j})\rangle.
    \]
    With this shift of the input \(x\), we have now removed the bias
    \(\bias_j\). In the remainder we operate on \(x-x_0\) as if
    on \(x\).

    In order to prove \eqref{eq: bound im by re}, we need
    an upper bound on the imaginary part and a lower bound of the real
    part. Let us start with a lower bound of the real part.
    For this we make crucial use of the assumption that \(|V_\tin|=1\)
    and thus that \(\weight_{\placeholder j}\in \complex\). This implies
    \(\langle x-x_0, \Re(\weight_{\placeholder j})\rangle =
    \Re(\weight_{\placeholder j})(x-x_0)\)
    and thus
    \begin{align}
    \nonumber
        |\Re(\bias_j + \langle x, \weight_{\placeholder j}\rangle)|
        &\ge |\Re(\weight_{\placeholder j})||x-x_0| 
        \\
    \nonumber
        &\ge |\Re(\weight_{\placeholder j}^*) - \Re(\weight_{\placeholder j}-\weight_{\placeholder j}^*)||x-x_0|
        \\
    \nonumber
        &\ge  (|\weight_{\placeholder j}^*| - \delta^\weight_j)|x-x_0|
        \\
    \label{eq: lower bound re}    
        \overset{\eqref{eq: delta w}}&\ge \frac{|\weight_{\placeholder j}^*|}2 |x-x_0|.
    \end{align}
    We now upper bound the imaginary part of \(\bias_j + \langle\weight_{\placeholder j}, x\rangle\), first at \(x_0\) where
    the real part does not loosen the bound, then at all remaining \(x\in
    \real\). Noting that \(\Im(\weight_{\placeholder j}^*)= \Im(\bias_j^*)=0\) we have at \(x_0\)
    \begin{align}
    \nonumber
        |\Im(\bias_j + \langle x_0, \weight_{\placeholder j} \rangle)|
        &\le  |\Im(\bias_j)| + |\Im(\weight_{\placeholder j})| \frac{|\Re(\bias_j)|}{|\Re(\weight_{\placeholder j})|}.
        \\
    \nonumber
        &\le |\Im(\bias_j-\bias_j^*)|
        + |\Im(\weight_{\placeholder j}-\weight_{\placeholder j}^*)| \frac{|\Re(\bias_j^*)| + |\Re(\bias_j-\bias_j^*)|}{|\Re(\weight_{\placeholder j}^*)| - |\Re(\weight_{\placeholder j}-\weight_{\placeholder j}^*)|}
        \\
    \nonumber
        &\le \delta^\bias_j + \delta^\weight_j \frac{|\bias^*_j| + \delta^\bias_j}{|\weight_{\placeholder j}^*| - \delta^\weight_j}
        \\
        \overset{\eqref{eq: delta bias}}&\le \frac{c_1}2 + \delta^\weight_j  \frac{1+2|\bias^*_j|}{|\weight_{\placeholder j}^*|/2}
        \overset{\eqref{eq: delta w}}\le c_1.
    \label{eq: upper bound im at x_0}
    \end{align}
    Using \(|V_\tin|=1\) again, the imaginary part is upper bounded by
    \begin{align*}
        |\Im(\bias_j + \langle x, \weight_{\placeholder j}\rangle)|
        &= |\Im\bigl(\bias_j + \langle x_0, \weight_{\placeholder j}\rangle
        + \langle x-x_0, \weight_{\placeholder j}\rangle\bigr)|
        \\
        &\le |\Im(\bias_n + \langle x_0, \weight_{\placeholder j} \rangle)|
        + \underbrace{|\Im(\weight_{\placeholder j})|}_{=|\Im\mathrlap{(\weight_{\placeholder j}-\weight_{\placeholder j}^*)| \le \delta^\weight_j}} |x - x_0|
        \\
        \overset{\eqref{eq: upper bound im at x_0}}&\le c_1 + c_1 \frac{|\weight_{\placeholder j}^*|}2 |x - x_0|
        \\
        \overset{\eqref{eq: lower bound re}}&\le c_1(1+ |\Re(\bias_j + \langle x, \weight_{\placeholder j}\rangle)|).
    \end{align*}
    This proves \eqref{eq: bound im by re} and therefore finishes the proof.
\end{proof}

\begin{lemma}[Real analytic response norm]
    \label{lem: real analytic response norm}
    Let a shallow neural network \(\network\) satisfy the assumptions
    \ref{res: response holomorphic} and \ref{res: response uniformly bounded}
    of Prop.~\ref{prop: holomorphic and bounded response}. Then, if \(X\) has finite \(2p\)-th
    moment, the function \(\param \mapsto \|\response_\param\|_{\Pr_X}^2\)
    is real analytic on the set of efficient parameters \(\efficient\).
\end{lemma}
\begin{proof}
    We prove the requirements of Morera's theorem \citep[e.g.][]{conwayFunctionsOneComplex1978,janichFunktionentheorie2004} which states that a
    function \(f:D\to\complex\) is holomorphic on an open set \(D\) if and only
    if for any triangular path \(\gamma\) in \(D\subseteq \complex\) we have
    \[
        \oint_\gamma f dz = 0.
    \]
    While Morera's theorem is defined for univariate holomorphic functions only,
    Osgood's Lemma \citep[e.g.][2]{gunningAnalyticFunctionsSeveral1965} states that
    a continuous function is holomorphic on an open set \(D\subseteq \complex^n\)
    if it is holomorphic in every variable separately. We therefore only need
    to apply Morea's theorem to every parameter individually.

    Since squares of holomorphic functions are holomorphic, we have that
    \(\param \mapsto (\response_\param(x))_l^2\) is holomorphic
    on an open neighborhood \(K_{\param_*}\) of any \(\param_*\in \efficient\) by \ref{res:
    response holomorphic} in Prop.~\ref{prop: holomorphic and bounded response}.
    Indexing the parameters \(\param\) with \(i\) and, by Osgood's Lemma, applying
    Morera's theorem to each parameter separately, we have for all triangular
    paths of \(\param_i\) contained in \(K_{\param_*}\)
    \begin{align*}
        \oint_\gamma \|\response_\param\|_{\Pr_X}^2 d\param_i
        &= \oint_\gamma \int \sum_{l\in V_\tout}(\response_\param(x))_l^2\; \Pr_X(dx) d\param_i
        \\
        \overset{\text{Fub.}}&= \int \sum_{l\in V_\tout} \underbrace{
            \oint_\gamma (\response_\param)_l^2(x) d\param_i
        }_{\underset{\text{Morea's thm.}}{\overset{\text{Prop.~\ref{prop: holomorphic and bounded response} \ref{res: response holomorphic}}}=}0} \Pr_X(dx)
        \\
        &= 0.
    \end{align*}
    To show the integrability necessary for the application of Fubini
    we use \ref{res: response uniformly bounded} of Prop.~\ref{prop: holomorphic
    and bounded response}, i.e.
    \[
        \oint_\gamma \sum_{l\in V_\tout} \int |(\response_\param(x))_l|^2 \Pr_X(dx) d\param_i
        \overset{\ref{res: response uniformly bounded}}\le \oint_\gamma \sum_{l\in V_\tout} C_l\; d\param_i< \infty,
    \]
    where the last inequality follows from the fact that \(\gamma\) is a path
    contained in \(K_{\param_*}\) and has bounded derivatives as a piecewise
    member of \(C^1\) \fxwarning{other argument for multivariate case?}.
\end{proof}

Now we check the requirements of this Proposition for specific activation functions
we use in Theorem~\ref{thm: morse function on efficient networks}.

\begin{theorem}
    \label{thm: analytic mean function}
    Let \(\network=(G, \activation, \param)\) be a shallow neural network
    with \(|V_\tin|=1\) and activation function \(\activation\in\{\sigmoid, \tanh\}\).
    Then the function \(\param \mapsto \|\response_\param\|_{\Pr_X}^2\) is
    real-analytic on on the set of efficient parameters \(\efficient\) for all
    random variables \(X\).
\end{theorem}
\begin{proof}
    We simply need to check the requirements \ref{assmpt: activation is
    holomorphic} and \ref{assmpt: activation grows at most with power p} for \(p=0\)
    to apply Proposition~\ref{prop: holomorphic and bounded response} and
    Lemma~\ref{lem: real analytic response norm}.  Since \(\tanh\) can be
    expressed with the \(\sigmoid\)
    activation function
    \begin{align*}
        \tanh(z)
        &= \frac{e^z - e^{-z}}{e^z + e^{-z}} 
        = \frac{1 - e^{-2z}}{1 + e^{-2z}}
        = \frac{1}{1+ e^{-2z}} - \frac{1}{e^{2z} + 1}
        \\
        &= \sigmoid(2z) - \sigmoid(-2z),
    \end{align*}
    it is sufficient to prove this claim for the sigmoid function and translate
    it to \(\tanh\) by an application of the triangle inequality
    \[
        |\tanh(z)| \le  2 |\sigmoid(2z)| \le 2c_2 \le \tilde{c}_2. 
    \]
    For \(\activation(x) = \sigmoid(x) = \frac1{1+e^{-x}}\) we use \(c_1 = \frac14\).
    So for \(z = x + \im y\in M\) we have
    \[
        |y| \le \frac14(1+|x|) \le \frac{\pi + |x|}4
    \]
    and we will prove that \(\activation\) is bounded by \(c_2 = 1/\sqrt{0.8}\). To do so we
    will prove that \(|1+e^{-z}|^2 \ge 0.8\) for all \(z\in M\).

    The following decomposition will be convenient:
    \begin{align}
    \nonumber
        |1+e^{-z}|^2
        &= |e^{-\im y} (e^{\im y} + e^{-x})|^2
        \\
    \nonumber
        &= |\cos(y) + \im \sin(y) + e^{-x}|^2
        = (e^{-x} + \cos(y))^2 + \sin^2(y)
        \\
        &= e^{-2x} + 2e^{-x}\cos(y) + 1
    \label{eq: representation I}
        \\ 
        &= e^{-x}(e^{-x} + 2\cos(y)) + 1
    \label{eq: representation II}
    \end{align}
    \begin{enumerate}
        \item \textbf{Case \(|x| \le \pi\):}
        In this case, we have \(|y| \le \frac{\pi}2\) and therefore \(\cos(y) \ge 0\).
        With representation \eqref{eq: representation I} this implies
        \(|1+e^{-z}|^2 \ge 1\).

        \item \textbf{Case \(x > \pi\):}
        We have \(|e^{-x} + 2\cos(y)| \le e^{-\pi} + 2 \le 2.2\)
        and \(|e^{-x}| \le 1/20\). Therefore by \eqref{eq: representation II}
        \[
            |1+e^{-z}|^2 \ge 1 - |e^{-x}| |e^{-x} + 2\cos(y)|
            \ge 1 - \frac{2.2}{20} \ge 0.8
        \]

        \item \textbf{Case \(x < -\pi\):}
        We have \(e^{-x} > e^{\pi} > 20\) and therefore by \eqref{eq: representation II}
        \[
            |1+e^{-z}|^2 \ge 20( 20 - 2 \cos(y)) + 1 \ge 1.
        \]
    \end{enumerate}
    So in all cases \(|1+ e^{-z}|^2 \ge 0.8\) and we have proven the bound.
    Since \(\sigmoid\) and \(\tanh\) are meromorphic functions, they are holomorphic
    everywhere except for their poles. In particular they are holomorphic on
    \(M\) where they are bounded.
\end{proof}



==> sections/clasification_diagram.tex <==
\begin{center}
\begin{NiceTabular}{ *{6}{c} }[corners, hvlines]
    \Block{1-6}{all possible parameters \(\param\)}\\
    \Block[borders=right]{1-2}{efficient} & & \Block{1-4}{redundant} & & & \\
    polynomially efficient & ? & Def.~\ref{def: efficient} \ref{it: disused neuron} & \Block{1-3}{Def.~\ref{def: efficient} \ref{it: linear combination of neurons}}\\
    & & \Block{1-3}{general redundancy} &&& \(\activation\)-specific \\
    & & \Block{2-1}{deactivation\\ \scriptsize(\(\weight_{j\placeholder}=0\))} & \Block{2-1}{bias\\\scriptsize(\(\weight_{\placeholder j}=0\))} & \Block{1-2}{generalized duplication} & \NotEmpty \\
    & & & \NotEmpty & duplication & \\
    \CodeAfter
        % \TikzEveryCell{offset=1pt,draw}
        \tikz \node[below=4em of 3-1, align=center,xshift=-2em] (isolated) {strongly convex minima\\ \& isolated crit.\ points\\ (\(|V_\tout|=1\), Theorem~\ref{thm: morse function on efficient networks})};
        \tikz \draw[-Stealth] ([yshift=-2pt]3-1.south) -- node[fill=white,align=center,text=black!70] {a.s.\\for MSE} (isolated) ;

        \tikz \node[below=9em of 3-2, align=center] (not_poly_efficient) {empty set\\ (Theorem~\ref{thm: characterization of efficient networks})};
        \tikz \draw[-Stealth] ([yshift=-2pt]3-2.south) -- node[near end,xshift=0.5em,fill=white,text=black!70] {\(\activation\in \{\substack{\sigmoid\\\tanh}\}\)} (not_poly_efficient);

        \tikz \node[below=11em of 6-4.south, align=center,xshift=-5em] (not_exists) {crit. points do not exist\\(Proposition~\ref{prop: bias red do not exist})};
        \tikz \draw[-Stealth] ([yshift=-2pt]6-4.south) -- node[near end,fill=white,align=center,text=black!70] {a.s. for MSE} (not_exists);

        \tikz \draw[decoration={brace,amplitude=5pt,raise=2.5em,mirror},line width=1pt,decorate]
        ([xshift=-5pt]5-3.west) -- node[above=-6em,align=center,fill=white] {minima never have strictly convex\\ neighborhoods (Theorem~\ref{thm: critical points of redundant type})} ([xshift=5pt]4-6.east |- 5-3.west);

        \tikz \draw[decoration={brace,amplitude=5pt,raise=6.5em,mirror},line width=1pt,decorate]
        ([xshift=-5pt]5-4.west) -- node[above=-10em,align=center] {critical points are never isolated\\(\(|V_\tout|=1\), Theorem~\ref{thm: critical points of redundant type})} ([xshift=5pt]4-6.east |- 5-3.west);

        % \tikz \node[below=5em of 5-6.south, anchor=north, align=center,xshift=-1em] (not_isolated) {crit. points never isolated\\(Theorem~\ref{thm: critical points of redundant type})};
        % \tikz \draw[-Stealth] ([yshift=-2pt]6-5.south) -- (not_isolated);
        % \tikz \draw[-Stealth] ([yshift=-2pt]5-6.south) -- node[fill=white,xshift=1em,text=black!70] {\(\activation\in \{\substack{\sigmoid\\\tanh}\}\)} (not_isolated);
\end{NiceTabular}%\rule[-3.5cm]{0pt}{0.4pt}
\end{center}
\vspace{6em}

==> sections/decomposition.tex <==






==> sections/main_results.tex <==
\section{Main results}

\begin{figure}
	\input{sections/clasification_diagram.tex}
	\caption{Classification of the parameter space of shallow neural networks}
	\label{fig: visualize_local_min}
\end{figure}

Our results are summarized in Figure~\ref{fig: visualize_local_min}.
We decompose the set of configurations in an efficient and redundant domain, see Definition~\ref{def: efficient}.

classify the possible parameters of a shallow neural network into
efficient and redundant parameters in Definition~\ref{def: efficient}.
Note that the set of efficient parameters is generally much larger than the
degeneration set of redundant parameters (e.g. Theorem~\ref{thm:
characterization of efficient networks}). In Theorem~\ref{thm: characterization
of efficient networks} we also show that the set of efficient parameters
(Definition~\ref{def: efficient}) coincides with the subset of polynomially
efficient parameters (Definition~\ref{def: polynomially efficient}) for the
activation functions \(\sigmoid\) and \(\tanh\).

This leads us to our main result (Theorem~\ref{thm: morse function on
efficient networks}) where we prove that the mean squared error (MSE) cost is a
Morse function on the space of polynomially efficient parameters for a wide
class of data distributions (characterized by Assumption~\ref{assmpt: data
distribution}). Critical points are therefore isolated and local minima
have strongly convex neighborhoods.

Having characterized the critical points in the set of polynomially efficient
parameters, we turn to the characterization of the degenerate case.
We prove in Theorem~\ref{thm: critical points of redundant type} that
redundant minima can never have a strictly convex neighborhood as
there is always a continuum of parameters of equal cost in the neighborhood.
We further show that this continuum is a continuum of critical points
for a subset of redundancy types, i.e. critical points are never isolated.
Note that this characterization of the set of redundant parameters
does not require any assumptions about the loss function or the data
distribution such as Assumption~\ref{assmpt: data distribution}.
With the help of Assumption~\ref{assmpt: data distribution}, we can additionally
almost surely rule out the sole existence of a certain type of redundancy: bias
redundancies (Proposition~\ref{prop:
bias red do not exist}). Conversely, we show that the other types of redundancies
cannot be ruled out to exist. We do so
by extending efficient critical points of smaller networks with these
redundancies to obtain critical points with these redundancies (Prop.~\ref{prop:
extending bias and deactivation}, Prop.~\ref{prop: extending duplication}).

In the previous sentence we implicitly assumed critical points of efficient
networks to exist. We thus prove in Theorem~\ref{thm: existence of efficient minima}
that any arbitrarily small open set of efficient parameters has a positive
probability to contain a minimum (and in particular a critical point).

\subsection{Classification of parameters}

In the following \(\network=(\mathbb V,\psi)\) is a fixed ANN.
We start by defining the class of efficient parameters. 

	
%	We note that the negation of condition \ref{it: linear combination of neurons} is equivalent to an `affine linear independence' of the
%	neurons \(j\in V_1\):  Indeed, condition \ref{it: linear combination of neurons} is not satisfiable if and only if the
%	equation
%	\[
%		\lambda_0 + \sum_{j\in V_1} \lambda_j
%		\activation\Bigl(\bias_j + \sum_{i\in V_0} x_i\weight_{ij}\Bigr)
%		= 0 
%	\]
%	has the unique solution \(\lambda_j = 0\) for all \(j \in V_1 \uplus \{0\}\).
%


For technical reasons we need to work with a stronger independence assumption as the one in \ref{it: linear combination of neurons}  of the former definition.
%In the following we will define a family of ``polynomially efficient''
%sets of parameters. It is straightforward to see that these sets are subsets of the efficient parameters
%since polynomial independence implies the affine linear independence condition
%required for efficiency.

% \begin{definition}[Polynomial independence]
% 	\label{def: polynomial independence} Let $n\in\nat_0$ and \(m=(m_{\emptyset}, m_0, \dots, m_n)\in\nat_0^{n+2}\).
% 	\begin{itemize}
% 	\item[(i)]
% 	%Let \(\network=(G, \activation, \param)\) be a shallow network and
%     A configuration \(\param\) is called \emph{\(m\)-polynomially
%     independent} if $\phi$ is
%     \(n\)-times differentiable and the equation
%     \[
%         0 = P^{(\emptyset)}(x)
%         + \sum_{j\in V_1}
%         \sum_{k=0}^n P^{(k)}_j(x) \activation^{(k)}\Bigl(\bias_j + \sum_{i\in V_0}x_i\weight_{ij} \Bigr) \quad \forall x\in \real^{V_0}
%     \]
%     considered in all polynomials  %implies \(P^{(k)}_j \equiv 0\) 
%     \(P^{(\emptyset)}\) and \((P^{(k)}_j:j\in V_1, k\in\{0,\dots,n\})\) of at most degree $m_\emptyset$ and  $m_k$, respectively, has the unique solution with all polynomials being identical zero.
%     %and \(P^{(\bias)}\), where the polynomials \(P^{(k)}_j\)
%     %are at most of degree \(m_k\).
%     Here, \(\activation^{(k)}\) denotes the \(k\)-th derivative of the activation function \(\activation\).
%     \item[(ii)] A configuration \(\theta\) is called \emph{$m$-polynomially
% 	efficient}, if 
% 	\begin{itemize}\item[(a)] all neurons are used and
% 	\item[(b)] it is \(m\)-polynomially     independent.
% 	\end{itemize}
% 	We denote by $\polyEfficient^m$ the set of all $m$-polynomially
% 	efficient configurations.
%     \end{itemize}
% \end{definition}

Obviously, a configuration is $(0,0)$-polynomially efficient if and only if it is efficient in the sense of Definition~\ref{def: efficient}. But in general the assumption of polynomial efficiency is stronger. 

As we will show next both notions generally coincide in the case where 
 the activation function is either \(\sigmoid\) or \(\tanh\)! %we show in
%the following theorem that the set of efficient and the sets of polynomially
%efficient parameters always coincide. 
Additionally, we provide an explicit set
representation.

% \begin{theorem}[Characterization of efficient networks for \(\sigmoid\) and \(\tanh\)]
%     \label{thm: characterization of efficient networks}
%     Assume that in the considered ANN \(\network\) the activation function  \(\activation\) is either  \(\sigmoid\) or \(\tanh\). Then for every \(n\in\nat_0\) and \(m=(m_{\emptyset}, m_0, \dots, m_n)\in\nat_0^{n+2}\)
%    one has
%    \[
%    \efficient=\polyEfficient^m=\efficient_0,
%    \]
%    where
%     \[
%             \efficient_0
%             = \Biggl\{
%                 \param =(\weight, \bias)\in \real^{E \times (V\setminus V_0)}:
%                 {
%                 \begin{aligned}[c]
%                     \scriptstyle \weight_{j\placeholder}
%                     &\scriptstyle\neq 0
%                     &&\scriptstyle \forall j \in V_1,
%                     \\[-0.5em]
%                     \scriptstyle\weight_{\placeholder j}
%                     &\scriptstyle\neq 0
%                     &&\scriptstyle\forall j\in V_1, 
%                     \\[-0.5em]
%                     \scriptstyle(\weight_{\placeholder i}, \bias_i)
%                     &\scriptstyle\neq \pm(\weight_{\placeholder j}, \bias_j)
%                     &&\scriptstyle\forall i,j\in V_1\text{ with }i\not=j
%                 \end{aligned}
%                 }
%             \Biggr\}
%         \]
%         is as in (\ref{??}).
% %
% %    \begin{enumerate}[label=\text{\normalfont(\roman*)}]
% %        \item\label{it: efficient} \(\param\) is efficient,
% %        \item\label{it: 0-redundant} \(\param\in \redundant_0^{G}\), where
% %        %\(\redundant_0^{\activation,G}\) is the open set of networks with zero
% %        %\(\activation\)-specific redundancies \fixme{Ich sehe nicht, wo $\psi$ eingeht.}
% %        \[
% %            \redundant_0^{\activation,G}
% %            := \Biggl\{
% %                \param =(\weight, \bias)\in \real^{E \times (V\setminus V_0)}:
% %                {
% %                \begin{aligned}[c]
% %                    \scriptstyle \weight_{j\placeholder}
% %                    &\scriptstyle\neq 0
% %                    &&\scriptstyle \forall j \in V_1,
% %                    \\[-0.5em]
% %                    \scriptstyle\weight_{\placeholder j}
% %                    &\scriptstyle\neq 0
% %                    &&\scriptstyle\forall j\in V_1, 
% %                    \\[-0.5em]
% %                    \scriptstyle(\weight_{\placeholder i}, \bias_i)
% %                    &\scriptstyle\neq \pm(\weight_{\placeholder j}, \bias_j)
% %                    &&\scriptstyle\forall i,j\in V_1\text{ with }i\not=j
% %                \end{aligned}
% %                }
% %            \Biggr\},
% %        \]
% %        where \(\weight_{j\placeholder}=(\weight_{jl})_{l\in V_\tout}\)  and
% %        similarly \(\weight_{\placeholder j} = (\weight_{ij})_{i\in V_\tin}\).
% %
% %        \item\label{it: polynomial independence} \(\param\) is \(m\)-polynomially efficient for every (or one) \(m\)
% %		with length \(n\ge 2\). %(i.e. \(m\) contains some \(m_\bias\) and \(m_0\)).
% %    \end{enumerate}
% \end{theorem}
\begin{proof}[Proofsketch] The proof is established by showing that $\efficient\subset \efficient_0\subset \polyEfficient^m\subset \efficient$. Note that $\polyEfficient^m\subset \efficient$ as indicated before.
\begin{itemize}
%	\item 	 the cycle \(\ref{it: efficient} \Rightarrow \ref{it: 0-redundant}
%	\Rightarrow \ref{it: polynomial independence} \Rightarrow \ref{it: efficient}\),
%	where the last implication ``\(\ref{it: polynomial independence} \Rightarrow
%	\ref{it: efficient}\)'' is trivial.
	\item
	To prove ``\(\efficient \subset \efficient_0\)''
	we will show that for every parameter $\param$  in \(\efficient_0^c\) is  not in \(\efficient\). More explicitly, we will construct a redundancy and show that one of the properties \ref{it: disused neuron} or \ref{it:  linear combination of neurons} does not hold.
	
	 %we have ``\(\neg\ref{it: 0-redundant}\Rightarrow \neg\ref{it: efficient}\)'', that is
	%for any parameter \(\param\) that is not in  \( \redundant_0^{\activation, G}\) we will
	%linearly combine a neuron or get the disuse of one neuron by definition.
	% This implication is split into two parts:
	% \begin{enumerate}
	% 	\item The requirements \emph{independent} of the activation function:
	% 	\begin{enumerate}
	% 		\item \(\weight_{j\placeholder}\neq 0\) follows directly from the
	% 		requirement that every neuron is used.  \(\weight_{j\placeholder} = 0\)
	% 		is a ``\emph{deactivation redundancy}''.

	% 		\item
	% 		\(\weight_{\placeholder j} \neq 0\) ensures that the neuron is not
	% 		constant which could be removed and moved into the bias.
	% 		\(\weight_{\placeholder j} = 0\) is a ``\emph{bias redundancy}''.


	% 		\item
	% 		\((\weight_{\placeholder i}, \bias_i) \neq (\weight_{\placeholder
	% 		j}, \bias_j)\) ensures that no two neurons have identical
	% 		parameters. \((\weight_{\placeholder i}, \bias_i) = (\weight_{\placeholder
	% 		j}, \bias_j)\) is a ``\emph{duplication redundancy}''.
	% 	\end{enumerate}

	% 	\item The requirements \emph{specific} to \(\activation\in \{\sigmoid,\tanh\}\).
	% 	This only includes
	% 	\((\weight_{\placeholder i}, \bias_i) \neq -(\weight_{\placeholder j}, \bias_j)\),
	% 	which follows from symmetries of these activation functions that allow
	% 	the reconstruction of the reflected neuron.
	% 	\((\weight_{\placeholder i}, \bias_i) = -(\weight_{\placeholder j}, \bias_j)\)
	% 	is an activation-function-specific ``\emph{sign symmetric redundancy}''.
	% \end{enumerate}

    \item
    It will be harder to prove that ``\(\efficient_0\subset \polyEfficient^m\)''
    and we will first consider the case with one dimensional input (i.e.
    \(\# V_\tin =1\)).  This proof relies on the complex poles of the meromorphic
    activation
    function \(\activation\in\{\sigmoid, \tanh\}\).  We will then show that generally the one-dimensional result also implies the general result. Here, we will not make again use of the assumption that  \(\activation\in\{\sigmoid, \tanh\}\). %that the one-dimensional
%    version implies the general version. 
%This strategy is most likely
  %  transferable to other activation functions (i.e.\ only the one dimensional
   % case needs to be considered and this implication applied), but since the set
   % defined in \ref{it: 0-redundant} is specific to the activation functions
   % \(\sigmoid\) and \(\tanh\) we cannot phrase it entirely independently.
    \qedhere
\end{itemize}
\end{proof}


\subsection{Analysis of critical points}


 
In this section we finally get to our main result: The mean
squared error (MSE) is almost surely a Morse function on the set of polynomially
efficient parameters. But the almost sure quantifier requires some
assumptions about the distribution of the data.

\begin{assumption}[Data distribution]
	\label{assmpt: data distribution}
	Assume
	\begin{enumerate}[label=\text{\normalfont (A\arabic*)}]
		\item\label{as: centered, universal, Gaussian target}
		the target function \(\rf\) is a centered, universal\footnote{
			A random function is `universal' if its covariance kernel 
			\(\C_\rf(x,y) = \cov(\rf(x), \rf(y))\) is universal. The kernel \(\C_\rf\) is universal,
			if its reproducing kernel hilbertspace (RKHS) is a subspace of the
			continuous functions (\(C_\rf\) is a `Mercer kernel'), and the RKHS
			is \emph{dense} in the space of continuous functions. Details in 
			Definition~\ref{def: universal} and
			\citep{carmeliVectorValuedReproducing2010}.
		} Gaussian random function,
		\item\label{as: P_X is constant} the input distribution \(\rP_X = \Pr(X\in \cdot \mid \rP_Z)\) is a constant, i.e. \(\rP_X \overset{\text{a.s.}}= \Pr_X\),
		\item\label{as: support of X contains open set} the support of \(\Pr_X\) contains an open set,
		\item\label{as: X compactly supported} \(X\) is compactly supported.
	\end{enumerate}
\end{assumption}

For this wide class of randomly chosen data distributions we get our result.
That is for the squared loss function \(\loss(\hat{y}, y) = \|\hat{y}- y\|^2\)
the induced MSE cost function is a Morse function on the set of
polynomially efficient parameters.


\begin{remark}
	The assumption of a compactly supported \(X\) \ref{as: X compactly
	supported} is only required to prove that \(\param\mapsto
	\|\response_\param\|_{\Pr_X}^2\) is (real) analytic.
	If \(\activation\in\{\sigmoid,\tanh\}\), then
	\begin{enumerate}
		\item \(\param\mapsto \|\response_\param\|_{\Pr_X}^2\) is (real)
		analytic if \(\# V_\tin=1\) (but not necessarily \(\# V_\tout=1\), see
		Theorem~\ref{thm: analytic mean function}).

		\item The set of efficient parameters is polynomially efficient
		(Theorem~\ref{thm: characterization of efficient networks}).
	\end{enumerate}
\end{remark}

We thus show that in the set of \((0,0,1,2)\)-polynomially efficient parameters there are
almost always only isolated critical points (Theorem~\ref{thm: morse function on
efficient networks}), moreover the cost function is almost surely a morse
function on the set of \((0,0,1,2)\)-polynomially efficient parameters.
For activation functions other than \(\activation\in\{\sigmoid,\tanh\}\) this
leaves a small gap: There may be a set of efficient parameters, which are not
polynomially efficient. Example~\ref{ex: softplus} provides an example for
how such a gap may look like.

It may seem surprising that we only need to make assumptions about the
distribution of the target function and not the distribution of the
entire relationship \(\rP_Z\). The reason for this is, that
for the MSE we have (Proposition~\ref{prop: decomposition})
\[
	\Cost(\phi)
	= \E\bigl[\|\phi(X) - \rf(X)\|^2 \mid \rP_Z\bigr]
	+ \E\bigl[\|\noise\|^2\mid \rP_Z\bigr].
\]
The above shows that the minimization of the MSE is independent of the
noise as it only changes the cost by a constant. Assumptions about the
distribution of the target function \(\rf\) are therefore sufficient
for the analysis of the optimization landscape.


\paragraph*{Do efficient/redundant critical points exist?}

This is the content of the following result, where we show that
any open set of efficient parameters contains a local minimum
(in particular a critical point) with positive probability.






==> sections/mse.tex <==
\section{Mean squared error}

While the theory on redundancies and the characterization of efficient networks
was completely deterministic, an analysis of the likelihood of isolated critical
points requires a probabilistic framework.


==> sections/polynomial_independence.tex <==
\subsection{Checking the polynomial independence assumption}

It is straightforward to check that the activation functions are real analytic with
complex singularities.\fxnote{more extensive proof anyway}

To check the polynomial independence property, we first use the series representation of
analytic functions to obtain an easy to verify condition and then check this
condition with the help of the computer algebra system \texttt{sympy}.

Using the series representation
\[
    \activation(x) = \sum_{k=0}^\infty a_k x^k   
\]
we have for polynomials \(P_n(x) = \sum_{k=0}^n p_{k,k} x^k\) and \(n\in\{0,1,2\}\)
\begin{alignat*}{3}
    \Psi(y) 
    &= P_0(y) \activation(y) && + P_1(y)\activation'(y) &&+ P_2(y)\activation''(y)
    \\
    &= P_0(y) \sum_{k=0}^\infty a_k y^k
    &&+ P_1(y) \sum_{k=1}^\infty a_kk y^{k-1}
    &&+ P_2(y) \sum_{k=2}^\infty a_k k(k-1) y^{k-2}
    \\
    &= \sum_{k=0}^\infty p_{0,0} a_k y^k
    &&
    \begin{aligned}[t]
        +& \sum_{k=1}^\infty p_{1,0} a_kk y^{k-1}
        \\
        +& \sum_{k=1}^\infty p_{1,1} a_kk y^k
    \end{aligned}
    &&
    \begin{aligned}[t]
    +& \sum_{k=2}^\infty p_{2,0} a_k k(k-1) y^{k-2}
    \\
    +& \sum_{k=2}^\infty p_{2,1} a_k k(k-1) y^{k-1}
    \\
    +& \sum_{k=2}^\infty p_{2,2} a_k k(k-1) y^k
    \end{aligned}
    \\
    &= \sum_{k=0}^\infty p_{0,0} a_k y^k
    &&
    \begin{aligned}[t]
        +& \sum_{k=0}^\infty p_{1,0} a_{k+1}(k+1) y^k
        \\
        +& \sum_{k=1}^\infty p_{1,1} a_kk y^k
    \end{aligned}
    &&
    \begin{aligned}[t]
    +& \sum_{k=0}^\infty p_{2,0} a_{k+2} (k+2)(k+1) y^k
    \\
    +& \sum_{k=1}^\infty p_{2,1} a_{k+1} (k+1)k y^k
    \\
    +& \sum_{k=2}^\infty p_{2,2} a_k k(k-1) y^k
    \end{aligned}
\end{alignat*}
where we applied an index shift in the last equation to ensure we have \(y^k\) everywhere.
\(\Psi(y)\) is therefore a power series with coefficients
\[
    c_k = \Biggl\langle \begin{pmatrix}
        a_k \\
        (k+1) a_{k+1}  \\
        k a_k \\
        (k+2)(k+1) a_{k+2} \\
        (k+1)k a_{k+1} \\
        k(k-1) a_k
    \end{pmatrix}, \begin{pmatrix}
        p_{0,0} \\
        p_{1,0} \\
        p_{1,1} \\
        p_{2,0} \\
        p_{2,1} \\
        p_{2,2}
    \end{pmatrix}
    \Biggr\rangle
    =: \langle \texttt{row}_k, p\rangle
\]
where we note that we can start the summation at \(k=0\) for all terms since we then have
zeros in the terms we left out previously.
Since \(\Psi \equiv 0\) implies \(c_k = 0\) for all \(k\)
it is sufficient to prove that a selection of rows \(\texttt{row}_k\) forming a
matrix \(M\) has rank \(6\), because then we have a fully determined system of
linear equations proving \(p=0\) is the unique solution and therefore
that \(\Psi = 0\) implies \(P_0=P_1=P_2=0\) (which is the polynomial independence property).

We prove this for the \texttt{softplus}, \texttt{logistic}, \texttt{tanh} and \texttt{GELU}
activation functions using the computer algebra system \texttt{sympy}. The
code we used follows below.

\inputminted[linenos,firstnumber=0]{python3}{code/polynomial_independence.py}

Running this script with \texttt{python3.11} and \texttt{sympy} version \texttt{1.12.1}
results in

\begin{center}
    \begin{verbatim}
    Checking polynomial independence property:
    ------------------------------------------
    softplus: True
    logistic: True
    gelu: True
    tanh: True
    \end{verbatim}
\end{center}

==> sections/representer_thm.tex <==
\section{Idea: Representer Theorem}

Needs \(\closure{\cH_\infty}\) to be RKHS.
\citep{scholkopfGeneralizedRepresenterTheorem2001}

If the support of \(X\) is finite (size \(n\)), result will be in \(\cH_n\) if the kernel
and \(\cH_n\) fit together.



==> sections/space_of_prediction_functions.tex <==
\section{Space of prediction functions}

For an activation function \(\sigma\) (e.g. ReLU, softplus),
we want to consider one hidden layer of size \(n\), i.e.
\[
    \cH_n
    = \Bigl\{
        f: x\mapsto \sum_{i=1}^n \varphi_i \circ \sigma \circ \psi_i(x) 
        \;:\; \varphi_i, \psi_i \text{ affine linear functions}, \|f\|_{\Pr_{X\mid \rf}} < \infty
    \Bigr\}
\]
now we consider the closure \(\overline{\cH_n}\) with respect to the norm
\(\|\cdot\|_{\Pr_{X\mid\rf}}\), e.g. for \(X\mid \rf \sim \uniform(0,1)\), the closure with respect to
\[
    \|f\|_{\Pr_{X\mid \rf}}^2 = \int_0^1 f^2(x) dx.
\]
Goal: We want to prove almost surely
\[
    \argmin_{f\in \closure{\cH^n}} \Cost(f) \subseteq \cH_n 
\]

\section{Idea: argmin may be viewed as Projection}
\[
    P(\rf)
    = \argmin_{f\in \closure{\cH_n}} \Cost(f)
    = \argmin_{f\in \closure{\cH_n}} \|f -\rf\|_{\Pr_{X\mid\rf}}^2
\]

\begin{lemma}
Let $H$ be a Hilbert space and $V$ a closed sub\textbf{space} of $H$. If $P\ :\ H \to V$, then the following two conditions are equivalent:
 
\begin{enumerate}
    \item $P$ is linear, $P^2 = P$, and $\ker P \perp V$.
    \item For all $x \in H, P(x) = \argmin_{y \in V} \|y - x\|$. 
\end{enumerate}
\end{lemma}
\begin{proof}
    \citep{sinclairCharacterizationProjectionOperator2016}
\end{proof}

\(\cH_\infty\) is a vector space equipped with a dot product (but not \(\cH_n\) for \(n<\infty\)).

Note that
\[
    \cH_{n, \psi}
    = \Bigl\{
        f: x\mapsto \sum_{i=1}^n \varphi_i \circ \sigma \circ \psi_i(x) 
        \;:\; \varphi_i\text{ affine linear functions}, \|f\|_{\Pr_{X\mid \rf}} < \infty
    \Bigr\}
\]
are vector spaces for \(\psi=(\psi_1,\dots, \psi_n)\) affine linear functions. So we can write
\[
    \cH_n
    = \bigcup_{\psi} \cH_{n, \psi}
\]
since
\[
    \bigcup_{\psi} \closure{\cH_{n, \psi}}
    \subseteq \closure{\cH_n}
\]
we have
\begin{align*}
    \min_{f\in \closure{\cH_n}} \Cost(f)
    &= \inf_{f\in \cH_n}\Cost(f)
    = \inf_{\psi} \min_{f\in \closure{\cH_{n,\psi}}} \Cost(f)
    \\
    &= \inf_{\psi} \Cost(P_\psi(\rf))
    \\
    &= \inf_{\psi} \|(1-P_\psi)\rf\|_{\Pr_{X\mid \rf}}^2
    = \inf_{\psi} \|\rf\|_{\Pr_{X\mid \rf}}^2
    - 2\langle \rf, P_\psi \rf\rangle_{\Pr_{X\mid \rf}}
    + \|P_\psi\rf\|_{\Pr_{X\mid \rf}}^2
    \\
    &=  \|\rf\|_{\Pr_{X\mid \rf}}^2 - \sup_{\psi}\| P_\psi\rf \|_{\Pr_{X\mid \rf}}^2
\end{align*}
where \(P_\psi\) is the projection to \(\closure{\cH_{n,\psi}}\), i.e. \(\ker P_\psi \perp \cH_{n,\psi}\).
We now have \(P_\psi \rf\) is \fxnote*{really? Does this work for linear
operators just like for linear maps?}{Gaussian}.
Since \(P_\psi\) is a \emph{continuous} linear operator as a projection,
integration can be exchanged with this linear operator, which implies
\[
    \E[P_\psi \rf(x)] = P_\psi \E[\rf(x)] = P_\psi \mu_\rf(x)
\]
similarly we have covariance
\[
    P_\psi \C_{\rf}(x,y) P_\psi^\transpose.
\]
